Watch out for This Commit! A Study of Influential Software Changes

One single code change can significantly influence a wide range of software systems and their users. For example, 1) adding a new feature can spread defects in several modules, while 2) changing an API method can improve the performance of all client programs. Developers often may not clearly know whether their or others' changes are influential at commit time. Rather, it turns out to be influential after affecting many aspects of a system later. This paper investigates influential software changes and proposes an approach to identify them early, i.e., immediately when they are applied. We first conduct a post-mortem analysis to discover existing influential changes by using intuitions such as isolated changes and changes referred by other changes in 10 open source projects. Then we re-categorize all identified changes through an open-card sorting process. Subsequently, we conduct a survey with 89 developers to confirm our influential change categories. Finally, from our ground truth we extract features, including metrics such as the complexity of changes, terms in commit logs and file centrality in co-change graphs, to build machine learning classifiers. The experiment results show that our prediction model achieves overall with random samples 86.8% precision, 74% recall and 80.4% F-measure respectively.

==> 05-experiment.tex <==
\section{Experiment Design}
\label{sec:experiment}

\subsection{Research Questions}
\label{sec:questions}

(What defines influential changes? --- post-mortem metrics)

RQ0: What is the key metric to determine "influential changes" here?

(What makes influential changes?)

RQ1: Are complex changes influential in the future? (internal complexity 
---> size, cyclomatic, etc --- and inter-class+external complexity ---> class coupling, fan-in/out)

RQ2: Are early changes influential? (historical metrics)

RQ3: Do popular developer make influential changes? (social metrics)

(Why are influential changes important?)

RQ4: Do influential changes affect the popularity of projects? (profit/social impact)

RQ5: Do influential changes make developer influential? (social impact)

RQ6: Who does benefit from it?






\subsection{Subjects}

\dongsun{In this time, it seems we can only adopt Linux kernel. However, we can
list up sub-modules in the kernel.}



\subsection{Identifying Influential Changes}

\subsubsection{Metrics}
\label{sec:metrics}
We manually look into each commit detected by our post-mortem analysis program
and analyze the importance of this commit:

\begin{enumerate}
    \item Is it a fix to a long standing bug?
    \item Does it introduce a new feature or interface?
    \item Does it introduce a potential issue?
    \item Does it contain something that requires attention of other developers/users?
\end{enumerate}

\subsubsection{Experiment Procedure}
\label{sec:procedure}
For each project, we firstly collect its data, including source code repository
and issue reports with user comments in its issue tracking system. After
preprocessing we extract interesting artifacts and store them in a database
for reuse and query.  Then we try to find commits that could be influential
using different post-mortem metrics, such as how long an issue is resolved
since being reported and how long a file is updated since a previous commit and
remains unchanged until a next commit.  These commits are then undergone a
manual evaluation of whether it is influential or not and assigned a label
accordingly.

\input{04-model}


\subsection{Qualitative Analysis}

\dongsun{this section describes how we did qualitative analysis. For example,
how we sampled some of influential changes.}


==> 06-results.tex <==
\section{Results}
\label{sec:results}




==> code/lgrindef <==
cocci:\
	:pb=\p\d?\(:cf:np=\)\d?;:bb={:be=}:\
	:cb=/*:ce=*/:sb=":se=\e":lb=':le=\e':\
	:tl:\
	:zb=@:ze=@:tb=%%:te=%%:mb=%\$:me=\$%:vb=%\|:ve=\|%:\
	:kw=identifier type expression parameter list != position ocaml script:


==> listing/kernel-after.tex <==
spin_lock_irqsave(&as->lock, flags);
if (!usbin_retire_desc(u, urb) &&
    u->flags & FLG_RUNNING &&
    !usbin_prepare_desc(u, urb) &&
    (suret = usb_submit_urb(urb,GFP_ATOMIC)) == 0) {
  u->flags |= mask;
} else {
  u->flags &= ~(mask | FLG_RUNNING);
  wake_up(&u->dma.wait);
  printk(KERN_DEBUG "...", suret);
}
spin_unlock_irqrestore(&as->lock, flags);

==> table/stats_blocking.tex <==
%\multirow{2}{*}{Safety hole} & \multicolumn{2}{c}{Number of exported functions collected in the } \\
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{lcc}
    Project Name & \# blocking issues & \# relevant changes\\
\toprule
{\tt Camel} & 73 & 332\\
{\tt Cassandra} & 31 & 37\\
{\tt commons-codec} & 2 & 26\\
{\tt commons-collections} & 6 & 12\\
{\tt commons-compress} & 3 & 7\\
{\tt commons-csv} & 2 & 5\\
{\tt commons-io} & 4 & 10\\
{\tt commons-lang} & 10 & 29\\
{\tt commons-math} & 10 & 38\\
{\tt hadoop} & 79 & 81\\
{\tt spring-framework} & 26 & 53\\
{\tt storm} & 4 & 40\\
{\tt wildfly} & 30 & 20\\
\bottomrule
{\tt Total} & 280 & 690\\
\bottomrule
\end{tabular}
}


==> table/storageproxy-isolated-commits.tex <==
\begin{table*}[t]
\centering
\caption{Isolated commits for ``StorageProxy.java'' in ``Cassandra'' project}
\begin{tabular}{|p{3cm}|p{1.5cm}|p{8cm}|}
\hline
File & Short hash & Commit message\\\hline
StorageProxy.java&97c022f&short circuits sending a message if the mutation's destination is the local node.  does not implement hint handling; takes the full message route if hints are involved.  patch by Sandeep Tata; reviewed by jbellis for CASSANDRA-132 \\\hline
StorageProxy.java&f6d0154&merge from 0.3 branch \\\hline
StorageProxy.java&3673e28&multitable support. \\\hline
StorageProxy.java&4e3a440&spelling fixes.  patch by Michael Greene; reviewed by jbellis for CASSANDRA-281 \\\hline
StorageProxy.java&dd1688c&merge from 0.4 branch \\\hline
StorageProxy.java&5e9b35c&rename getMessagingInstance -> instance; r/m unused methods from FBUtiltities patch by jbellis; reviewed by Eric Evans for CASSANDRA-385 \\\hline
StorageProxy.java&9cc51b5&fix range queries and Range/Bounds intersections.  patch by jbellis; tested by Jack Culpepper for CASSANDRA-781 \\\hline
StorageProxy.java&0095f0c&CASSANDRA-625 switch to slf4j logging. Patch by Gabriele Renzi, reviewed by Gary Dusbabek. \\\hline
StorageProxy.java&c5e97fd&improve DEBUG logging of insert path.  patch by Ryan King and jbellis for CASSANDRA-1023 \\\hline
StorageProxy.java&7c9191f&merge from 0.6 \\\hline
StorageProxy.java&d8755b3&clean up of TokenMetadata and ARS.  patch by mdennis; reviewed by jbellis for CASSANDRA-1194 \\\hline
StorageProxy.java&aa95d4a&always repair on digest mismatch for CL > 1.  patch by jbellis \\\hline
StorageProxy.java&389bac7&merge from 0.6 \\\hline
\end{tabular}
\label{tab:StorageProxy-isolated-commits}
\end{table*}


==> table/ten_fold.tex <==
\centering
\resizebox{1\linewidth}{!}{
\begin{tabular}{l l c | c | c c c | c c c}
  \multirow{2}{*}{\bf Project Name} & 
  \multirow{2}{*}{\bf Metrics} &
  \multirow{2}{*}{\bf Machine Learner} &
  \multirow{2}{*}{\bf Accurary} &
  \multicolumn{3}{c|}{\bf Influential Class} & 
  \multicolumn{3}{c|}{\bf None Influential Class} \\
  & & & & Precision & Recall & F-Measure & Precision & Recall & F-Measure \\

\toprule
{\tt codec}
& CC & NB & 95.3 & 100.0 & 87.5 & 93.3 & 93.1 & 100.0 & 96.4 \\
& CC & RF & 93.0 & 100.0 & 81.2 & 89.7 & 90.0 & 100.0 & 94.7 \\
& CM & NB & 93.0 & 88.2 & 93.8 & 90.9 & 96.2 & 92.6 & 94.3 \\
& CM & RF & 86.0 & 85.7 & 75.0 & 80.0 & 86.2 & 92.6 & 89.3 \\
& CS & NB & 65.1 & 66.7 & 12.5 & 21.1 & 65.0 & 96.3 & 77.6 \\
& CS & RF & 67.4 & 56.2 & 56.2 & 56.2 & 74.1 & 74.1 & 74.1 \\
& CC CM & NB & 93.0 & 93.3 & 87.5 & 90.3 & 92.9 & 96.3 & 94.5 \\
& CC CM & RF & 86.0 & 91.7 & 68.8 & 78.6 & 83.9 & 96.3 & 89.7 \\
& CC CS & NB & 90.7 & 92.9 & 81.2 & 86.7 & 89.7 & 96.3 & 92.9 \\
& CC CS & RF & 88.4 & 92.3 & 75.0 & 82.8 & 86.7 & 96.3 & 91.2 \\
& CM CS & NB & 86.0 & 81.2 & 81.2 & 81.2 & 88.9 & 88.9 & 88.9 \\
& CM CS & RF & 90.7 & 100.0 & 75.0 & 85.7 & 87.1 & 100.0 & 93.1 \\
& ALL & NB & 90.7 & 83.3 & 93.8 & 88.2 & 96.0 & 88.9 & 92.3 \\
& ALL & RF & 90.7 & 92.9 & 81.2 & 86.7 & 89.7 & 96.3 & 92.9 \\
{\tt collections}
& CC & NB & 74.1 & 85.7 & 70.6 & 77.4 & 61.5 & 80.0 & 69.6 \\
& CC & RF & 79.6 & 87.1 & 79.4 & 83.1 & 69.6 & 80.0 & 74.4 \\
& CM & NB & 81.5 & 81.6 & 91.2 & 86.1 & 81.2 & 65.0 & 72.2 \\
& CM & RF & 83.3 & 85.7 & 88.2 & 87.0 & 78.9 & 75.0 & 76.9 \\
& CS & NB & 50.0 & 57.8 & 76.5 & 65.8 & 11.1 & 5.0 & 6.9 \\
& CS & RF & 79.6 & 81.1 & 88.2 & 84.5 & 76.5 & 65.0 & 70.3 \\
& CC CM & NB & 81.5 & 80.0 & 94.1 & 86.5 & 85.7 & 60.0 & 70.6 \\
& CC CM & RF & 90.7 & 93.9 & 91.2 & 92.5 & 85.7 & 90.0 & 87.8 \\
& CC CS & NB & 81.5 & 87.5 & 82.4 & 84.8 & 72.7 & 80.0 & 76.2 \\
& CC CS & RF & 79.6 & 81.1 & 88.2 & 84.5 & 76.5 & 65.0 & 70.3 \\
& CM CS & NB & 85.2 & 82.5 & 97.1 & 89.2 & 92.9 & 65.0 & 76.5 \\
& CM CS & RF & 87.0 & 90.9 & 88.2 & 89.6 & 81.0 & 85.0 & 82.9 \\
& ALL & NB & 83.3 & 79.1 & 100.0 & 88.3 & 100.0 & 55.0 & 71.0 \\
& ALL & RF & 96.3 & 97.1 & 97.1 & 97.1 & 95.0 & 95.0 & 95.0 \\
{\tt compress}
& CC & NB & 59.3 & 43.8 & 77.8 & 56.0 & 81.8 & 50.0 & 62.1 \\
& CC & RF & 63.0 & 0.0 & 0.0 & 0.0 & 65.4 & 94.4 & 77.3 \\
& CM & NB & 85.2 & 85.7 & 66.7 & 75.0 & 85.0 & 94.4 & 89.5 \\
& CM & RF & 74.1 & 100.0 & 22.2 & 36.4 & 72.0 & 100.0 & 83.7 \\
& CS & NB & 63.0 & 40.0 & 22.2 & 28.6 & 68.2 & 83.3 & 75.0 \\
& CS & RF & 81.5 & 70.0 & 77.8 & 73.7 & 88.2 & 83.3 & 85.7 \\
& CC CM & NB & 81.5 & 83.3 & 55.6 & 66.7 & 81.0 & 94.4 & 87.2 \\
& CC CM & RF & 74.1 & 100.0 & 22.2 & 36.4 & 72.0 & 100.0 & 83.7 \\
& CC CS & NB & 74.1 & 58.3 & 77.8 & 66.7 & 86.7 & 72.2 & 78.8 \\
& CC CS & RF & 81.5 & 75.0 & 66.7 & 70.6 & 84.2 & 88.9 & 86.5 \\
& CM CS & NB & 85.2 & 85.7 & 66.7 & 75.0 & 85.0 & 94.4 & 89.5 \\
& CM CS & RF & 81.5 & 83.3 & 55.6 & 66.7 & 81.0 & 94.4 & 87.2 \\
& ALL & NB & 81.5 & 83.3 & 55.6 & 66.7 & 81.0 & 94.4 & 87.2 \\
& ALL & RF & 74.1 & 100.0 & 22.2 & 36.4 & 72.0 & 100.0 & 83.7 \\
{\tt csv}
& CC & NB & 74.1 & 66.7 & 72.7 & 69.6 & 80.0 & 75.0 & 77.4 \\
& CC & RF & 66.7 & 62.5 & 45.5 & 52.6 & 68.4 & 81.2 & 74.3 \\
& CM & NB & 88.9 & 100.0 & 72.7 & 84.2 & 84.2 & 100.0 & 91.4 \\
& CM & RF & 88.9 & 100.0 & 72.7 & 84.2 & 84.2 & 100.0 & 91.4 \\
& CS & NB & 70.4 & 71.4 & 45.5 & 55.6 & 70.0 & 87.5 & 77.8 \\
& CS & RF & 81.5 & 75.0 & 81.8 & 78.3 & 86.7 & 81.2 & 83.9 \\
& CC CM & NB & 85.2 & 88.9 & 72.7 & 80.0 & 83.3 & 93.8 & 88.2 \\
& CC CM & RF & 85.2 & 100.0 & 63.6 & 77.8 & 80.0 & 100.0 & 88.9 \\
& CC CS & NB & 77.8 & 77.8 & 63.6 & 70.0 & 77.8 & 87.5 & 82.4 \\
& CC CS & RF & 70.4 & 66.7 & 54.5 & 60.0 & 72.2 & 81.2 & 76.5 \\
& CM CS & NB & 88.9 & 100.0 & 72.7 & 84.2 & 84.2 & 100.0 & 91.4 \\
& CM CS & RF & 92.6 & 100.0 & 81.8 & 90.0 & 88.9 & 100.0 & 94.1 \\
& ALL & NB & 85.2 & 88.9 & 72.7 & 80.0 & 83.3 & 93.8 & 88.2 \\
& ALL & RF & 85.2 & 100.0 & 63.6 & 77.8 & 80.0 & 100.0 & 88.9 \\
{\tt io}
& CC & NB & 84.2 & 80.0 & 66.7 & 72.7 & 85.7 & 92.3 & 88.9 \\
& CC & RF & 86.8 & 88.9 & 66.7 & 76.2 & 86.2 & 96.2 & 90.9 \\
& CM & NB & 92.1 & 80.0 & 100.0 & 88.9 & 100.0 & 88.5 & 93.9 \\
& CM & RF & 94.7 & 100.0 & 83.3 & 90.9 & 92.9 & 100.0 & 96.3 \\
& CS & NB & 55.3 & 41.4 & 100.0 & 58.5 & 100.0 & 34.6 & 51.4 \\
& CS & RF & 71.1 & 53.8 & 58.3 & 56.0 & 80.0 & 76.9 & 78.4 \\
& CC CM & NB & 92.1 & 80.0 & 100.0 & 88.9 & 100.0 & 88.5 & 93.9 \\
& CC CM & RF & 89.5 & 100.0 & 66.7 & 80.0 & 86.7 & 100.0 & 92.9 \\
& CC CS & NB & 97.4 & 92.3 & 100.0 & 96.0 & 100.0 & 96.2 & 98.0 \\
& CC CS & RF & 92.1 & 90.9 & 83.3 & 87.0 & 92.6 & 96.2 & 94.3 \\
& CM CS & NB & 94.7 & 91.7 & 91.7 & 91.7 & 96.2 & 96.2 & 96.2 \\
& CM CS & RF & 89.5 & 100.0 & 66.7 & 80.0 & 86.7 & 100.0 & 92.9 \\
& ALL & NB & 94.7 & 85.7 & 100.0 & 92.3 & 100.0 & 92.3 & 96.0 \\
& ALL & RF & 92.1 & 100.0 & 75.0 & 85.7 & 89.7 & 100.0 & 94.5 \\
{\tt lang}
& CC & NB & 81.9 & 91.9 & 70.8 & 80.0 & 75.4 & 93.5 & 83.5 \\
& CC & RF & 77.7 & 74.5 & 85.4 & 79.6 & 82.1 & 69.6 & 75.3 \\
& CM & NB & 72.3 & 72.0 & 75.0 & 73.5 & 72.7 & 69.6 & 71.1 \\
& CM & RF & 87.2 & 95.0 & 79.2 & 86.4 & 81.5 & 95.7 & 88.0 \\
& CS & NB & 48.9 & 50.0 & 20.8 & 29.4 & 48.6 & 78.3 & 60.0 \\
& CS & RF & 63.8 & 63.0 & 70.8 & 66.7 & 65.0 & 56.5 & 60.5 \\
& CC CM & NB & 76.6 & 74.1 & 83.3 & 78.4 & 80.0 & 69.6 & 74.4 \\
& CC CM & RF & 90.4 & 93.3 & 87.5 & 90.3 & 87.8 & 93.5 & 90.5 \\
& CC CS & NB & 89.4 & 95.2 & 83.3 & 88.9 & 84.6 & 95.7 & 89.8 \\
& CC CS & RF & 87.2 & 86.0 & 89.6 & 87.8 & 88.6 & 84.8 & 86.7 \\
& CM CS & NB & 74.5 & 73.1 & 79.2 & 76.0 & 76.2 & 69.6 & 72.7 \\
& CM CS & RF & 87.2 & 97.4 & 77.1 & 86.0 & 80.4 & 97.8 & 88.2 \\
& ALL & NB & 77.7 & 75.5 & 83.3 & 79.2 & 80.5 & 71.7 & 75.9 \\
& ALL & RF & 86.2 & 90.7 & 81.2 & 85.7 & 82.4 & 91.3 & 86.6 \\
{\tt math}
& CC & NB & 81.2 & 69.6 & 57.1 & 62.7 & 84.6 & 90.4 & 87.4 \\
& CC & RF & 90.1 & 87.5 & 75.0 & 80.8 & 90.9 & 95.9 & 93.3 \\
& CM & NB & 80.2 & 59.1 & 92.9 & 72.2 & 96.5 & 75.3 & 84.6 \\
& CM & RF & 90.1 & 100.0 & 64.3 & 78.3 & 88.0 & 100.0 & 93.6 \\
& CS & NB & 71.3 & 40.0 & 7.1 & 12.1 & 72.9 & 95.9 & 82.8 \\
& CS & RF & 70.3 & 43.8 & 25.0 & 31.8 & 75.3 & 87.7 & 81.0 \\
& CC CM & NB & 78.2 & 57.5 & 82.1 & 67.6 & 91.8 & 76.7 & 83.6 \\
& CC CM & RF & 91.1 & 100.0 & 67.9 & 80.9 & 89.0 & 100.0 & 94.2 \\
& CC CS & NB & 83.2 & 72.0 & 64.3 & 67.9 & 86.8 & 90.4 & 88.6 \\
& CC CS & RF & 91.1 & 91.3 & 75.0 & 82.4 & 91.0 & 97.3 & 94.0 \\
& CM CS & NB & 75.2 & 53.1 & 92.9 & 67.5 & 96.2 & 68.5 & 80.0 \\
& CM CS & RF & 91.1 & 100.0 & 67.9 & 80.9 & 89.0 & 100.0 & 94.2 \\
& ALL & NB & 77.2 & 56.1 & 82.1 & 66.7 & 91.7 & 75.3 & 82.7 \\
& ALL & RF & 91.1 & 100.0 & 67.9 & 80.9 & 89.0 & 100.0 & 94.2 \\
{\tt spr}
& CM & NB & 88.6 & 93.8 & 88.2 & 90.9 & 80.6 & 89.3 & 84.7 \\
& CM & RF & 87.3 & 97.7 & 82.4 & 89.4 & 75.0 & 96.4 & 84.4 \\
& CS & NB & 46.8 & 73.7 & 27.5 & 40.0 & 38.3 & 82.1 & 52.3 \\
& CS & RF & 82.3 & 83.6 & 90.2 & 86.8 & 79.2 & 67.9 & 73.1 \\
& CM CS & NB & 84.8 & 89.8 & 86.3 & 88.0 & 76.7 & 82.1 & 79.3 \\
& CM CS & RF & 87.3 & 95.6 & 84.3 & 89.6 & 76.5 & 92.9 & 83.9 \\
{\tt storm}
& CC & NB & 71.9 & 82.4 & 70.0 & 75.7 & 60.0 & 75.0 & 66.7 \\
& CC & RF & 90.6 & 100.0 & 85.0 & 91.9 & 80.0 & 100.0 & 88.9 \\
& CM & NB & 75.0 & 87.5 & 70.0 & 77.8 & 62.5 & 83.3 & 71.4 \\
& CM & RF & 93.8 & 100.0 & 90.0 & 94.7 & 85.7 & 100.0 & 92.3 \\
& CS & NB & 59.4 & 81.8 & 45.0 & 58.1 & 47.6 & 83.3 & 60.6 \\
& CS & RF & 62.5 & 66.7 & 80.0 & 72.7 & 50.0 & 33.3 & 40.0 \\
& CC CM & NB & 84.4 & 85.7 & 90.0 & 87.8 & 81.8 & 75.0 & 78.3 \\
& CC CM & RF & 93.8 & 100.0 & 90.0 & 94.7 & 85.7 & 100.0 & 92.3 \\
& CC CS & NB & 71.9 & 82.4 & 70.0 & 75.7 & 60.0 & 75.0 & 66.7 \\
& CC CS & RF & 93.8 & 100.0 & 90.0 & 94.7 & 85.7 & 100.0 & 92.3 \\
& CM CS & NB & 84.4 & 85.7 & 90.0 & 87.8 & 81.8 & 75.0 & 78.3 \\
& CM CS & RF & 87.5 & 90.0 & 90.0 & 90.0 & 83.3 & 83.3 & 83.3 \\
& ALL & NB & 75.0 & 83.3 & 75.0 & 78.9 & 64.3 & 75.0 & 69.2 \\
& ALL & RF & 90.6 & 100.0 & 85.0 & 91.9 & 80.0 & 100.0 & 88.9 \\
{\tt wfly}
& CM & NB & 87.1 & 96.0 & 88.9 & 92.3 & 50.0 & 75.0 & 60.0 \\
& CM & RF & 96.8 & 96.4 & 100.0 & 98.2 & 100.0 & 75.0 & 85.7 \\
& CS & NB & 58.1 & 93.8 & 55.6 & 69.8 & 20.0 & 75.0 & 31.6 \\
& CS & RF & 90.3 & 90.0 & 100.0 & 94.7 & 100.0 & 25.0 & 40.0 \\
& CM CS & NB & 87.1 & 96.0 & 88.9 & 92.3 & 50.0 & 75.0 & 60.0 \\
& CM CS & RF & 96.8 & 96.4 & 100.0 & 98.2 & 100.0 & 75.0 & 85.7 \\
\bottomrule
\end{tabular}
}


==> table/ten_fold_nb.tex <==
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l l | c c c | c c c}
  \multirow{2}{*}{\bf Project Name} & 
  \multirow{2}{*}{\bf Metrics} &
  \multicolumn{3}{c|}{\bf Influential Class} & 
  \multicolumn{3}{c}{\bf None Influential Class} \\
  & & Precision & Recall & F-Measure & Precision & Recall & F-Measure \\

\toprule

{\tt Commons-codec}
& CC & 94.1 & 80.0 & 86.5 & 78.9 & 93.8 & 85.7 \\
& CM & 95.2 & 100.0 & 97.6 & 100.0 & 93.8 & 96.8 \\
& CS & 85.7 & 15.0 & 25.5 & 47.7 & 96.9 & 63.9 \\
& CC CM & 92.9 & 97.5 & 95.1 & 96.7 & 90.6 & 93.5 \\
& CC CS & 94.3 & 82.5 & 88.0 & 81.1 & 93.8 & 87.0 \\
& CM CS & 93.0 & 100.0 & 96.4 & 100.0 & 90.6 & 95.1 \\
& ALL & 92.9 & 97.5 & 95.1 & 96.7 & 90.6 & 93.5 \\
\midrule
{\tt Commons-collections}
& CC & 100.0 & 73.2 & 84.5 & 69.4 & 100.0 & 82.0 \\
& CM & 80.9 & 92.7 & 86.4 & 84.2 & 64.0 & 72.7 \\
& CS & 60.7 & 90.2 & 72.5 & 20.0 & 4.0 & 6.7 \\
& CC CM & 82.6 & 92.7 & 87.4 & 85.0 & 68.0 & 75.6 \\
& CC CS & 97.1 & 82.9 & 89.5 & 77.4 & 96.0 & 85.7 \\
& CM CS & 78.0 & 95.1 & 85.7 & 87.5 & 56.0 & 68.3 \\
& ALL & 90.7 & 95.1 & 92.9 & 91.3 & 84.0 & 87.5 \\
\midrule
{\tt Commons-compress}
& CC & 86.2 & 92.6 & 89.3 & 87.5 & 77.8 & 82.4 \\
& CM & 84.4 & 100.0 & 91.5 & 100.0 & 72.2 & 83.9 \\
& CS & 59.5 & 92.6 & 72.5 & 33.3 & 5.6 & 9.5 \\
& CC CM & 84.4 & 100.0 & 91.5 & 100.0 & 72.2 & 83.9 \\
& CC CS & 67.6 & 92.6 & 78.1 & 75.0 & 33.3 & 46.2 \\
& CM CS & 84.4 & 100.0 & 91.5 & 100.0 & 72.2 & 83.9 \\
& ALL & 84.4 & 100.0 & 91.5 & 100.0 & 72.2 & 83.9 \\
\midrule
{\tt Commons-csv}
& CC & 46.2 & 54.5 & 50.0 & 70.6 & 63.2 & 66.7 \\
& CM & 88.9 & 72.7 & 80.0 & 85.7 & 94.7 & 90.0 \\
& CS & 83.3 & 45.5 & 58.8 & 75.0 & 94.7 & 83.7 \\
& CC CM & 77.8 & 63.6 & 70.0 & 81.0 & 89.5 & 85.0 \\
& CC CS & 70.0 & 63.6 & 66.7 & 80.0 & 84.2 & 82.1 \\
& CM CS & 77.8 & 63.6 & 70.0 & 81.0 & 89.5 & 85.0 \\
& ALL & 100.0 & 72.7 & 84.2 & 86.4 & 100.0 & 92.7 \\
\midrule
{\tt Commons-io}
& CC & 93.1 & 81.8 & 87.1 & 80.6 & 92.6 & 86.2 \\
& CM & 94.3 & 100.0 & 97.1 & 100.0 & 92.6 & 96.2 \\
& CS & 63.3 & 93.9 & 75.6 & 81.8 & 33.3 & 47.4 \\
& CC CM & 91.7 & 100.0 & 95.7 & 100.0 & 88.9 & 94.1 \\
& CC CS & 93.1 & 81.8 & 87.1 & 80.6 & 92.6 & 86.2 \\
& CM CS & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
& ALL & 97.1 & 100.0 & 98.5 & 100.0 & 96.3 & 98.1 \\
\midrule
{\tt Commons-lang}
& CC & 94.7 & 75.0 & 83.7 & 71.4 & 93.8 & 81.1 \\
& CM & 84.1 & 95.8 & 89.6 & 92.1 & 72.9 & 81.4 \\
& CS & 62.5 & 83.3 & 71.4 & 50.0 & 25.0 & 33.3 \\
& CC CM & 82.7 & 93.1 & 87.6 & 87.2 & 70.8 & 78.2 \\
& CC CS & 95.4 & 86.1 & 90.5 & 81.8 & 93.8 & 87.4 \\
& CM CS & 84.1 & 95.8 & 89.6 & 92.1 & 72.9 & 81.4 \\
& ALL & 82.4 & 97.2 & 89.2 & 94.3 & 68.8 & 79.5 \\
\midrule
{\tt Commons-math}
& CC & 89.9 & 82.4 & 86.0 & 81.6 & 89.4 & 85.3 \\
& CM & 81.8 & 100.0 & 90.0 & 100.0 & 74.5 & 85.4 \\
& CS & 51.3 & 73.1 & 60.3 & 39.6 & 20.2 & 26.8 \\
& CC CM & 90.0 & 100.0 & 94.7 & 100.0 & 87.2 & 93.2 \\
& CC CS & 88.0 & 81.5 & 84.6 & 80.4 & 87.2 & 83.7 \\
& CM CS & 90.0 & 100.0 & 94.7 & 100.0 & 87.2 & 93.2 \\
& ALL & 89.3 & 100.0 & 94.3 & 100.0 & 86.2 & 92.6 \\
\midrule
{\tt Spring-framework}
& CM & 92.2 & 86.4 & 89.2 & 77.3 & 86.4 & 81.6 \\
& CS & 65.2 & 95.5 & 77.5 & 37.5 & 5.1 & 9.0 \\
& CM CS & 92.7 & 91.8 & 92.2 & 85.0 & 86.4 & 85.7 \\
\midrule
{\tt Storm}
& CC & 92.8 & 71.9 & 81.0 & 74.7 & 93.7 & 83.1 \\
& CM & 93.3 & 93.3 & 93.3 & 92.4 & 92.4 & 92.4 \\
& CS & 90.0 & 50.6 & 64.7 & 62.7 & 93.7 & 75.1 \\
& CC CM & 93.0 & 74.2 & 82.5 & 76.3 & 93.7 & 84.1 \\
& CC CS & 92.5 & 69.7 & 79.5 & 73.3 & 93.7 & 82.2 \\
& CM CS & 91.5 & 96.6 & 94.0 & 95.9 & 89.9 & 92.8 \\
& ALL & 93.4 & 79.8 & 86.1 & 80.4 & 93.7 & 86.5 \\
\midrule
{\tt Wildfly}
& CM & 78.5 & 94.7 & 85.8 & 92.2 & 70.8 & 80.1 \\
& CS & 58.8 & 96.3 & 73.0 & 85.2 & 24.1 & 37.5 \\
& CM CS & 90.5 & 94.2 & 92.3 & 93.2 & 88.9 & 91.0 \\

\bottomrule
\end{tabular}
}

